Access Control Synthesis for Physical Spaces

Access-control requirements for physical spaces, like office buildings and airports, are best formulated from a global viewpoint in terms of system-wide requirements. For example, "there is an authorized path to exit the building from every room." In contrast, individual access-control components, such as doors and turnstiles, can only enforce local policies, specifying when the component may open. In practice, the gap between the system-wide, global requirements and the many local policies is bridged manually, which is tedious, error-prone, and scales poorly. We propose a framework to automatically synthesize local access control policies from a set of global requirements for physical spaces. Our framework consists of an expressive language to specify both global requirements and physical spaces, and an algorithm for synthesizing local, attribute-based policies from the global specification. We empirically demonstrate the framework's effectiveness on three substantial case studies. The studies demonstrate that access control synthesis is practical even for complex physical spaces, such as airports, with many interrelated security requirements.

==> generic-requirements.tex <==
\subsection{Generic Requirements}

\label{generic-requirements-formalization}

In this section we illustrate the formalization of two generic requirements: deadlock-freeness and deny-by-default.

\para{Deadlock-freeness}
%
Given a resource structure, we can formalize a global requirement stipulating that there are no deadlock resources. 
%
Formally, let ~$S = ({\cal R}, E, r, L)$ be a resource structure. The deadlock-freeness requirement for $S$ is:
%
\[ {\sf true}\Rightarrow {\sf AG}\ {\sf EX}\ {\sf true}~. \]
%
This requirement applies to all access requests. The access constraint ${\sf AG}\ {\sf EX}\ {\sf true}$ states that for any resource a subject can access, there is a resource that the subject can access next.
%
%Note that since~$\mathcal{R}$ is a finite set,~$\mathsf{id}\in \mathcal{R}$ can be written as the disjunction of finitely many equalities.
%%
A resource structure~$S$ and a configuration $c$ satisfy this requirement iff for any access requests $q\in {\cal Q}$, $S_{c,q}$ has no deadlock resources.

\para{Deny-by-default}
We first define positive and negative requirements. Let $S$ be a resource structure.
We write $C_S$ for the set of all configurations for~$S$.  
The set~$C_S$ is partially ordered under the relation $\sqsubseteq_S$, defined as:~$c\sqsubseteq_S c'$ iff $c(e)\subseteq c'(e)$, for any edge~$e$ of~$S$ and any two configurations~$c$ and~$c'$. 
%
Let $c$ and $c'$ be two configurations for a resource structure~$S$.
%
A requirement $T\Rightarrow \varphi$ is \emph{positive} iff $S,c\Vdash (T\Rightarrow \varphi)$ and $c \sqsubseteq c'$ imply  $S,c'\Vdash (T\Rightarrow \varphi)$.
%
A requirement $T\Rightarrow \varphi$ is \emph{negative} iff $S,c\Vdash (T\Rightarrow \varphi)$ and $c' \sqsubseteq c$ imply  $S,c'\Vdash (T\Rightarrow \varphi)$.
%
Intuitively, if a configuration satisfies a positive (negative) requirement, then any more (less) permissive configuration also satisfies the requirement. Although not all requirements are positive or negative, most real-world requirements are, including the requirements specified using our requirement patterns.


%
The deny-by-default requirement is defined relative to a set of positive requirements.  Let $S = ({\cal R}, E, r, L)$ be a resource structure, $R$ a set of requirements for $S$ that contains only
positive and negative requirements, and let $\{T_1\Rightarrow \varphi), \cdots, T_n\Rightarrow \varphi_n\}$ be the set of all positive requirements contained in $R$. 
%
The deny-by-default requirement for $R$ is
%
\[ \neg (T_1\vee \cdots \vee T_n)\Rightarrow \textsc{Deny}\ ({\sf id} \neq r)~. \]
%
Here we assume that $L(r)({\sf id}) = r$, i.e. the entry resource $r$ is labeled with its identifier $r$. Note that we use the deny pattern to formalize deny-by-default.

This requirement states that if none of the positive requirements are applicable to a request, then 
only the entry space is accessible to the subject who makes such a request.
%%
Adding deny-by-default to our running example's requirements would ensure that an intern cannot access, e.g., the meeting room.

==> problem.tex <==
\section{Policy Synthesis Problem}
\label{sec:problem}
We first describe our system model, and then formalize it. Afterward,
we formally define the policy synthesis problem.

\subsection{Formal Setting}
%
Below we formalize our system model, including attributes, resource
structures, policies, and requirements. In our formal model, 
%%we
%%identify the physical space that contains a protected resource with
%%the resource. That is, 
we do not distinguish between physical spaces and protected resources.
This modeling choice avoids unnecessary cluttering, without limiting
the reach and scope of our results. 

\para{Attributes}
%
We fix a finite set~$\cal A$ of \emph{attributes} and an infinite
set~$\cal V$ of attribute {\em values}. Each attribute $a\in {\cal A}$
is associated with a (possibly infinite) set of values. We partition
the set of attributes into subject attributes~${\cal A}_S$, contextual
attributes~${\cal A}_C$, and resource attributes~${\cal A}_R$.  An
{\em access request} is a total function mapping subject and
contextual attributes to values, and we denote the set of all access
requests by~${\cal Q}$. A {\em resource valuation} is a total function
that maps resource attributes to their values.
%%%
We refer to the pair~$(\mathcal{A},\mathcal{V})$ as the attribute
signature.


Two remarks are due here. First, in contrast to, e.g.,
XACML~\cite{xacml3}, an
access request in our setting does not refer to the resource
attributes.
This is because in our systems model, each PDP controls access to one
physical space. Since, as mentioned above, a PDP ``knows'' the space
under its control, there is no need to include resource attributes in
access requests.
%%
Second, we assume that subject attributes and contextual attributes do
not change in the course of making a policy decision. We relegate
discussing such attribute changes to~\secref{}.

%% This is a
%% practical assumption.
%% %%
%%   For instance, 
%% %%practically-relevant access control requirements do
%% %%  not consdier 
%% the effects of revoking a subject's attributes while the subject walks
%% from an office to another.


\para{Resource Structures}
%
A \emph{resource structure} is a tuple~$S = ({\cal R}, E, I, L)$,
where ${\cal R}$ is a set of {\em resources}, $E\subseteq {\cal
R}\times {\cal R}$ is a reflexive relation, $I\subseteq {\cal R}$ is a
set of \emph{entry resources}, and $L: {\cal R}\to ({\cal A}_R\to
{\cal V})$ is a total function mapping resources to resource
valuations. 
%
An example of a resource structure is given in
Figure~\ref{fig:synth-overview}. For simplicity we omit the self
edges, which connect a node to itself, when depicting resource
structures.
%
Any edge represents an enforcement point. 
%%
A resource structure constrains how subjects access resources: A
subject can directly access only the entry resources, while all the
remaining resources are accessed along paths starting from an entry
resource. 
%%
After a subject has accessed a resource, then the subject may access
the resource indefinitely. For example, a subject who accesses a room
can remain there indefinitely. This motivates the self edges, which we
assume permit all requests.



%
%% \textcolor{red}{not here} In \secref{sec:lang}, we define an expressive language
%% that can capture relevant requirements. Afterward, in
%% \secref{sec:synthesis}, we present a sound and complete algorithm for
%% synthesizing policies from requirements expressed in our language.

